SCOPE: A Self-supervised Framework for Improving Faithfulness in Conditional Text Generation

Large Language Models (LLMs), when used for conditional text generation, often produce hallucinations, i.e., information that is unfaithful or not grounded in the input context. This issue arises in typical conditional text generation tasks, such as text summarization and data-to-text generation, where the goal is to produce fluent text based on contextual input. When fine-tuned on specific domains, LLMs struggle to provide faithful answers to a given context, often adding information or generating errors. One underlying cause of this issue is that LLMs rely on statistical patterns learned from their training data. This reliance can interfere with the model's ability to stay faithful to a provided context, leading to the generation of ungrounded information. We build upon this observation and introduce a novel self-supervised method for generating a training set of unfaithful samples. We then refine the model using a training process that encourages the generation of grounded outputs over unfaithful ones, drawing on preference-based training. Our approach leads to significantly more grounded text generation, outperforming existing self-supervised techniques in faithfulness, as evaluated through automatic metrics, LLM-based assessments, and human evaluations.

==> tables/datasets_details.tex <==
\begin{table}[h]
\centering
\caption{Dataset Splits for ToTTo, FeTaQa, E2E, and WebNLGg}
\label{tab:dataset-splits}
\begin{tabular}{lrrrr}
\toprule
\multirow{2}{*}{Dataset} & \multicolumn{3}{c}{Split} & \multirow{2}{*}{Total} \\
\cmidrule(lr){2-4}
& Train & Validation & Test & \\
\midrule
totto & 123,456 & 10,000 & 10,000 & 143,456 \\
fetaqa & 80,000 & 10,000 & 10,000 & 100,000 \\
e2e & 42,061 & 5,467 & 6,755 & 54,283 \\
webnlg & 18,102 & 2,267 & 2,461 & 22,830 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/noisy_samples.tex <==
\begin{table*}[h]
\centering
\begin{tabular}{|m{0.1\textwidth}|m{0.8\textwidth}|}
\hline
input & \texttt{name[Green Man], priceRange[less than £20], area[riverside], familyFriendly[yes]} \\ \hline
reference  & Located near the river, Green Man is a family friendly place that offers \redhl{cheap sushi}. \\ \hline
$\alpha = 0.0$   & Located near riverside Green Man offers low-priced food in a family friendly environment. \\ \hline
$\alpha = 0.3$   & Green Man \redhl{Gaming} offers low prices and a great family friendly environment on their site in addition to their riverside location. \\ \hline
$\alpha = 0.6$   & \# Greenwoods is in the riverside district \redhl{and the suburb is named Green Manor. 1 out of 10 customers would recommend this product as it was not up to their standards.} The prices are \redhl{very high and they do not have a variety of products}. Children \redhl{are not allowed in this store.} \\ \hline
\end{tabular}
\caption{Noisy generation given structured context from E2E dataset. Facts highlighed in \redhl{red} denote hallucinations. In this example, even the reference exhibits hallucination.}
\label{tab:noisy-samples}
\end{table*}
